Challenges in Double Beta Decay

After nearly 80 years since the first guess on its existence, neutrino still escapes our insight: the mass and the true nature (Majorana or Dirac) of this particle is still unknown. In the past ten years, neutrino oscillation experiments have finally provided the incontrovertible evidence that neutrinos mix and have finite masses. These results represent the strongest demonstration that the Standard Model of electroweak interactions is incomplete and that new Physics beyond it must exist. None of these experimental efforts could however shade light on some of the basic features of neutrinos. Indeed, absolute scale and ordering of the masses of the three generations as well as charge conjugation and lepton number conservation properties are still unknown. In this scenario, a unique role is played by the Neutrinoless Double Beta Decay searches: these experiments can probe lepton number conservation, investigate the Dirac/Majorana nature of the neutrinos and their absolute mass scale (hierarchy problem) with unprecedented sensitivity. Today Neutrinoless Double Beta Decay faces a new era where large scale experiments with a sensitivity approaching the so-called degenerate-hierarchy region are nearly ready to start and where the challenge for the next future is the construction of detectors characterized by a tonne-scale size and an incredibly low background, to fully probe the inverted-hierarchy region. A number of new proposed projects took up this challenge. These are based either on large expansions of the present experiments or on new ideas to improve the technical performance and/or reduce the background contributions. n this paper, a review of the most relevant ongoing experiments is given. The most relevant parameters contributing to the experimental sensitivity are discussed and a critical comparison of the future projects is proposed.

==> 04-enr.tex <==



==> 05-bkg.tex <==
\subsection{Considerations on Sensitivity and Backgrounds}
\label{sec:expbac}

Any extraneous energy deposit in the detector near the \BBz Q-value limits the sensitivity to \mnu. Thus, any radioactive isotope with a Q-value greater than the \BBz end-point may be a potential background. Because the number of radioactive isotopes decreases with increasing Q, it is desirable to select a double beta decay candidate with as large a Q-value as possible. 
Beta- and alpha-emitting decays are easy to shield and thus are a problem only if they occur within the detector or on its surface. Penetrating gamma rays pose a more difficult problem.
In this subsection, we consider the origin of various sources of background and some techniques for their mitigation.

Natural radioactivity is present in all materials at some level. The source and detector must be very low in such impurities. Furthermore, the detector must be shielded from the environment and its associated radioactivity. This shielding must also be radio- pure. Because the total radioactivity of an impure material scales as its volume, it is usually an advantage to minimize the detector size. 
This can be most readily accomplished when the detector also serves as the source.
Cosmogenic activities build up in materials through nuclear reactions of cosmic ray muons and their secondary products, especially neutrons. These can be a significant background contribution both for the source and for the shielding material.
Some materials have no long-lived isotopes and thus have a built-in safeguard against cosmogenics. For experiments that must fight this problem, fabricating the apparatus underground and storing materials underground can greatly reduce this background. Unlike solid sources, a gaseous or liquid source can be continuously purified of such impurities.

